Compact Multi-level Sparse Neural Networks with Input Independent Dynamic Rerouting

Deep neural networks (DNNs) have shown to provide superb performance in many real life applications, but their large computation cost and storage requirement have prevented them from being deployed to many edge and internet-of-things (IoT) devices. Sparse deep neural networks, whose majority weight parameters are zeros, can substantially reduce the computation complexity and memory consumption of the models. In real-use scenarios, devices may suffer from large fluctuations of the available computation and memory resources under different environment, and the quality of service (QoS) is difficult to maintain due to the long tail inferences with large latency. Facing the real-life challenges, we propose to train a sparse model that supports multiple sparse levels. That is, a hierarchical structure of weights are satisfied such that the locations and the values of the non-zero parameters of the more-sparse sub-model area subset of the less-sparse sub-model. In this way, one can dynamically select the appropriate sparsity level during inference, while the storage cost is capped by the least sparse sub-model. We have verified our methodologies on a variety of DNN models and tasks, including the ResNet-50, PointNet++, GNMT, and graph attention networks. We obtain sparse sub-models with an average of 13.38% weights and 14.97% FLOPs, while the accuracies are as good as their dense counterparts. More-sparse sub-models with 5.38% weights and 4.47% of FLOPs, which are subsets of the less-sparse ones, can be obtained with only 3.25% relative accuracy loss.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tex/discussions.tex <==
\section{Discussions}

\subsection{Discussion on more than two levels of sparsity}
We use two-level sparsity to demonstrate our ``tiny-dense-small'' training methodology. In practice, two-level sparsity has demonstrated a good  trade-off between accuracy and DNN complexity.
In order to obtain more than 2 levels, we can generalize the training method to ``micro-dense-tiny-dense-small'' for triple-level sparsity, where the ``micro'' sub-model can be 3 to 4 times smaller than the tiny one. 3 to 4 times difference between adjacent sparsity levels makes a reasonable trade-off between accuracy and complexity. 

\subsection{Comparison to existing dynamic DNNs}
Several recent works \cite{wang2018skipnet,yu2019slimmable,yang2019condconv,ma2020weightnet} focus on \cross{``conditional''} \fei{``input dependent''} dynamic inference, i.e., which path to inference is determined by individual \cross{input samples} \fei{input, } where \fei{the} ``easy'' inputs go through simple paths and thus reduce computation\cross{s} on average. A fundamental difference of our ``dynamic rerouting'' is that ours is {input independent}, i.e., {any} input \cross{sample} \fei{data} can be switched from small to tiny sub-model from {any} designated switching point\cross{s} (e.g., 4 points for ResNet50). The switch\fei{ing} decision is based on run-time status such as \cross{current} \fei{the} latency before each switch\fei{ing} point, independent of \cross{samples} \fei{the input data}. Input independent rerouting is much simpler and more practical than \fei{the} NN based conditional rerouting in existing literature\fei{s}.
Second, our DNN models are much more sparse than the existing works. For example, our tiny ResNet50 has 5\% of weights of a dense counterpart, while SkipNet \cite{wang2018skipnet} has 88\%. Slimmable neural network \cite{yu2019slimmable} has one result \cross{on 27.06\% weights (and 1.4\% less accurate than our tiny ResNet50)} \fei{that achieves 1.4\% {\em less} accuracy than our tiny ResNet50 with 5$\times$ parameters (27.06\% vs 5.43\%)}. CondConv \cite{yang2019condconv} or WeightNet \cite{ma2020weightnet} \cross{is} \fei{are} even larger than the dense ResNet50.

\subsection{The reason of using ADMM on weight pruning} 
Any pruning method can be used such as magnitude-based, L1-regularization based, etc. We use ADMM \cross{as a tool} \fei{algorithm} because it enables dynamic penalty on the weights \cross{that}. 
\fei{Thus, it} receive\fei{s} higher accuracy than \fei{the} fixed regularization method\fei{s}, in particular \cross{for} \fei{at} large sparsity (i.e., tiny sub-models). As a result, we achieve the state-of-the-art accuracy for the presented sparsity levels. As a comparison, if one uses magnitude-based pruning, the accuracy of the tiny ResNet50 is only 68\%. Using ADMM, we presented the tiny ResNet50 with 73.60\% for the same setting.

